DreamLoop: Controllable Cinemagraph Generation from a Single Photograph

Cinemagraphs, which combine static photographs with selective, looping motion, offer unique artistic appeal. Generating them from a single photograph in a controllable manner is particularly challenging. Existing image-animation techniques are restricted to simple, low-frequency motions and operate only in narrow domains with repetitive textures like water and smoke. In contrast, large-scale video diffusion models are not tailored for cinemagraph constraints and lack the specialized data required to generate seamless, controlled loops. We present DreamLoop, a controllable video synthesis framework dedicated to generating cinemagraphs from a single photo without requiring any cinemagraph training data. Our key idea is to adapt a general video diffusion model by training it on two objectives: temporal bridging and motion conditioning. This strategy enables flexible cinemagraph generation. During inference, by using the input image as both the first- and last- frame condition, we enforce a seamless loop. By conditioning on static tracks, we maintain a static background. Finally, by providing a user-specified motion path for a target object, our method provides intuitive control over the animation's trajectory and timing. To our knowledge, DreamLoop is the first method to enable cinemagraph generation for general scenes with flexible and intuitive controls. We demonstrate that our method produces high-quality, complex cinemagraphs that align with user intent, outperforming existing approaches.

==> figures/extra.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/extra.pdf}
    % \vspace{-3mm}
    \caption{{\bf Fine Grained Controls .} (top) \textbf{Timing controls:} Highlights a scenario where timing control is essential for realistic motion. User intends to simulate the bead osciallting in simple harmonic motion (SHM). Without timing control, i.e., equally space points (top-left) the bead has constant motion, not following SHM, thus looking unrealistic. With timining control, user can assign more time the extrema and lesser time at the minima of SHM, accurately simulating physically realistic motion. (bottom) \textbf{Full vs. Partial motion paths:} Demonstrate 2 scenarios of the same example, where the user can either provide the full motion path (bottom-left) or just the initial motion trajectory (bottom-right) and remaining is automatically generated with our model. Corresponding video results are provided in supplementary material.}
    \lblfig{extra}
% \vspace{-2mm}
\end{figure}

==> figures/teaser.tex <==
% Preamble
% \usepackage{graphicx}
% \usepackage{xcolor}
% \usepackage{animate}

% Sizing knobs
\newlength{\cellw}
\newlength{\cellh}
\newlength{\rowgap}
\setlength{\cellw}{0.21\textwidth} % width of each small cell on the right
\setlength{\cellh}{5.2cm}           % height of each small cell
\setlength{\rowgap}{0.6em}          % vertical gap between right rows
\setlength{\tabcolsep}{0pt}         % remove tabular inner padding
\setlength{\fboxrule}{0.8pt}
\setlength{\fboxsep}{0pt}
\setkeys{Gin}{draft=false}          % ensure images render

\begin{figure*}[!t]
\centering
\begin{tabular}[t]{@{} c @{\hspace{0.8em}} c @{}} % left + right blocks, top-aligned
  % Left tall panel (height = 2*cellh + rowgap)
  \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \includegraphics[width=\linewidth,
                     height=\dimexpr 2\cellh + \rowgap\relax,
                     keepaspectratio]{images/teaser/teaser-p1.pdf}
  \end{minipage}
  &
  % Right: 2 x 3 grid
  \begin{tabular}[t]{@{} c @{\hspace{0.6em}} c @{\hspace{0.6em}} c @{}} 
    % Row 1
    \begin{minipage}[t]{\cellw}
      \vspace{0pt}
      \includegraphics[width=\linewidth,height=\cellh,keepaspectratio]{images/teaser/teaser1.png}
    \end{minipage} &
    \begin{minipage}[t]{\cellw}
      \vspace{0pt}
      \fcolorbox{black}{white}{%
        \animategraphics[autoplay,loop,width=\linewidth]{24}{images/teaser/teaser-1/}{0}{71}%
      }
    \end{minipage} &
    \begin{minipage}[t]{\cellw}
      \vspace{0pt}
      \includegraphics[width=\linewidth,height=\cellh,keepaspectratio]{images/teaser/teaser-p2.pdf}
    \end{minipage} \\[\rowgap]
    % Row 2
    \begin{minipage}[t]{\cellw}
      \vspace{0pt}
      \includegraphics[width=\linewidth,height=\cellh,keepaspectratio]{images/teaser/teaser2.png}
    \end{minipage} &
    \begin{minipage}[t]{\cellw}
      \vspace{0pt}
      \fcolorbox{black}{white}{%
        \animategraphics[autoplay,loop,width=\linewidth]{24}{images/teaser/teaser-2/}{0}{119}%
      }
    \end{minipage} &
    \begin{minipage}[t]{\cellw}x
      \vspace{0pt}
      \fcolorbox{black}{white}{%
        \animategraphics[autoplay,loop,width=\linewidth]{24}{images/teaser/teaser-3/}{0}{71}%
      }
    \end{minipage}
  \end{tabular}
\end{tabular}

\vspace{0.5em}
\caption{\textbf{Combined Results.} Left: prominent example. Right: six results in a 2×3 grid.}
\label{fig:combined_results_layout}
\end{figure*}

% \maketitle
